Diplomat: A conversational agent framework for goal-oriented group discussion

Recent work in human-computer interaction has explored the use of conversational agents as facilitators for group goal-oriented discussions. Inspired by this work and by the apparent lack of tooling available to support it, we created Diplomat, a Python-based framework for building conversational agent facilitators. Diplomat is designed to support simple specification of agent functionality as well as customizable integration with online chat services. We document a preliminary user study we conducted to help inform the design of Diplomat. We also describe the architecture, capabilities, and limitations of our tool, which we have shared on GitHub.

==> 5FutureWork_old.tex <==
\section{Future Work}
\label{sec:FutureWork}

Though we chose to focus on specific features in our experiment and in implementing Diplomat, We recognize many additional features that could enhance a chatbot.  

A chatbot in a meeting will require a set of rules that it responds to in order to optimize the outcome of the meetings. Since it is unclear what each group or person considers an optimal value of a meeting, we could use an agenda set by the user who creates the meeting to dictate the chatbot rules. In a simple agenda, the meeting host or members could specify the topics to be addressed and preferred time spent on each topic. With this information, a chatbot might be able to more easily interact to ensure the meeting is on track by responding to the changes in conversation. A chatbot could add value to these meetings by providing additional resources and recognizing the sentiment of the users. This proposed chatbot component will be most useful for meetings with predefined options and an agenda. A meeting that might follow this pattern could be a resume review. For example, each candidate’s resume is discussed for 5 minutes before comparing and contrasting them all for the last 10 minutes.  

We make many assumptions about the behavior of meeting participants and the ability for chatbots to influence an outcome. A chatbot could guide a discussion in a productive direction by recognizing the sentiment of each participant and prompt users to shift conversation in a productive direction. We hypothesize that people will get sidetracked or avoid coming to a decision to adhere to social norms. This means that rather than disagreeing with a person or group of people and making an assertive decision, people may linger on unimportant details to avoid social  disagreement. It is difficult to tell someone else that their idea is not good. The chatbot could address people individually or as a group. For example, as a group, if the time spent on a subtopic is nearing the specified time, the chatbot can warn the group that they need to move on. This strategy can be implemented using Topic Modeling and sentiment analysis, allowing the chatbot to recognize the topics that are being discussed and comparing them to the topics specified by the user. Additionally, if the group is nearing the allotted time in deciding a simple decision, the chatbot could suggest the majority rule, or the decision of a specified authority member to make the decision. The success of a chatbot in these conversations can initially be measured by how well the users stick to the proposed agenda.


Topic Modeling and Sentiment Analysis are two key NLP models to aid this chatbot. Using Topic Modeling, a chatbot could recognize when the group is off topic and suggests that the group shifts the conversation or even provides relevant papers to the topic. Using Sentiment Analysis, the bot might be able to recognize the general sentiment of each user. If conversations are taking too long or if there is discourse in a conversation, the bot can recognize the sentiment of the majority and either suggest the majority decision, or privately call out the person in the minority. This idea is similar to one proposed in the Neem Project \cite{barthelmess2005neem}, where “if a particular participant is expressing wishes that disagree with the rest of the group, [a chatbot] communicates in private with this participant, letting him or her know that the rest of the group seems to think differently.” Overall, by utilizing both Topic Modeling and Sentiment Analysis in a chatbot, unnecessary dissonance and divergence from the conversation can be detected and avoided. The image below demonstrates the bot recognizing dissenting opinions and providing a relevant topic to the conversation, aiming to manage the direction of the conversation. 

However, we consider two studies supporting the idea that Topic Modeling methods described above are unable to train well on small amounts of data \cite{hong2010empirical}. Studies support the idea that though Topic Modeling is a useful Natural Language Processing model to analyze texts, the brevity of documents in forums such as Twitter make analysis using Topic Modeling difficult, concluding that the models yield best results when initially trained on longer documents, posing restrictions on implementing Topic Modeling in live conversations \cite{hong2010empirical,alvarez2016topic}.

Finally, we speculate that priming is an important idea regarding the use of chatbots in decision-making conversations. A chatbot with priming features could be most useful in free-form discussions or a brainstorming session. A bot could prime a user in two ways- asking the right questions so that a user is prompted appropriately and teaching a user to act a certain way in conversation. Based on \cite{reitter2010priming}, when users use a word in their dialog, they are more likely to use that word again. From this, we gather that a chatbot can spur questions, priming users to discuss relevant topics and stimulate more discussion while brainstorming. Additionally, papers by \cite{isbister2000helper} and \cite{rienks2009pro} support the idea that when users know that a bot is about to correct them, they will automatically correct themselves before the bot can do it. We hypothesize that if a chatbot can prime users into knowing that when they speak too much, the chatbot will call them out in front of the group, they may reserve themselves more and allow for others to contribute. 

There are many options of exploration for virtual participants to aid decision-making scenarios. Allowing users to set an agenda allows a chatbot to intervene appropriately, ensuring the meeting remains within the preferred time and disagreements are settled using the predetermined tools (for example, majority). By intervening, the chatbot has the potential to provide new, relevant information, avoid social dissonance, and suggest courses of action if a discussion is no longer productive. Using Topic Modeling and Sentiment Analysis, a chatbot is able to recognize any opposition within the meeting and provide relevant topics and papers that will aid the structure of the meeting. Though some of these scenarios have been tested, the goal of the experiment we conducted is to use a chatbot to ease social dissonance in discussion and optimize the outcome of meeting decisions. 

